The Higgs transverse momentum distribution in gluon fusion as a multiscale problem

We consider Higgs production in gluon fusion and in particular the prediction of the Higgs transverse momentum distribution. We discuss the ambiguities affecting the matching procedure between fixed order matrix elements and the resummation to all orders of the terms enhanced by $\log(p_T^H/m_H)$ factors. Following a recent proposal (Grazzini et al., hep-ph/1306.4581), we argue that the gluon fusion process, computed considering two active quark flavors, is a multiscale problem from the point of view of the resummation of the collinear singular terms. We perform an analysis at parton level of the collinear behavior of the $\mathcal{O}(\alpha_s)$ real emission amplitudes; relying on the collinear singularities structure of the latter, we derive an upper limit to the range of transverse momenta where the collinear approximation is valid. This scale is then used as the value of the resummation scale in the analytic resummation framework or as the value of the $h$ parameter in the POWHEG-BOX code. A variation of this scale can be used to generate an uncertainty band associated to the matching procedure. Finally, we provide a phenomenological analysis in the Standard Model, in the Two Higgs Doublet Model and in the Minimal Supersymmetric Standard Model. In the two latter cases, we provide an ansatz for the central value of the matching parameters not only for a Standard Model-like Higgs boson, but also for heavy scalars and in scenarios where the bottom quark may play the dominant role.

==> helicityapp.tex <==
\section{Helicity amplitude for \texorpdfstring{$gg \to Hg$}{gg to Hg}}

\begin{figure}
  \centering
  \includegraphics[width=0.49\textwidth]{figures/combined-ampl-mh-125.pdf} \includegraphics[width=0.49\textwidth]{figures/combined-ampl-mh-500.pdf}
  \caption{Squared matrix element of the four helicity amplitudes for a light, $m_H = 125$ GeV (left) and for a heavy, $m_H = 500$ GeV Higgs boson.}
  \label{fig:amplcoll:all}
\end{figure}


In fig. \ref{fig:amplcoll:all} we plot all the four squared helicity amplitudes that we are considering,
as a function of $\pth$, to appreciate their relative importance, in the case of $m_H = 125$ GeV and $m_H = 500$ GeV.
For these two plots, the contributions of the top and the bottom quark were added together.
We observe that $\mathampl^{+++}$ dominates with respect to the other helicities.

%% taken from the SM phenomenology analysis
 The amplitude $\mathampl^{+++}$ and $\mathampl^{++-}$ receive significant corrections from the regular part,
starting from $\pth \simeq 140$ GeV. The amplitude $\mathampl^{-++}$ is dominated by the regular part, for both top and bottom quarks, while the amplitude $\mathampl^{-+-}$ is regular in the collinear limit
and therefore does not need to studied. The correction due to the regular part has the same signs for $\mathampl^{+++}$ and for $\mathampl^{++-}$ and tends to add in the sum of the squared helicity amplitudes.
In this case, the relevant scale at which the regular corrections become important which is suggested by the individual amplitudes, is close to the one derived by the sum over helicities ({\color{red} caso? spiegare?})
(cfr fig. \ref{fig:amplcoll:regall}).
In figure \ref{fig:amplcoll:regall} we repeat the comparison between the exact matrix element summed over helicities and its collinear approximation. We observe that the regular term become important with respect to
the collinear ones for a value of $\pth \simeq 90(120)$ GeV for a light (heavy) Higgs. 

From this study we can draw three remarks. First of all, the scale at which the collinear approximation fails is conservatively indicated by the analysis of the individual helicity amplitudes and is of
$\mathcal{O}(50)$ GeV in the case of a light Higgs and of $\mathcal{O}(130)$ GeV for a heavy Higgs. Secondly, the amplitude $\mathampl^{+++}$ is numerically dominant, 
but the precise value at the scale at which the collinear approximation fails strongly depends also on the contribution of the other amplitudes. Moreover, the scale suggested by the analysis
of the full amplitude that includes top and bottom contribution expresses the failure of the collinear approximation due to the top squared, bottom squared  and top-bottom interference terms.
One might also be interested to adopt a different approach, where the effects due to the top quark squared amplitudes are treated separately from those due to the bottom-top interference and to the
bottom squared amplitude, using the scales that emerge in the individual only-top and only-bottom amplitudes. The phenomenological impact can then be appreciated at hadron level,
after the inclusion of resummation effects.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pth"
%%% End: 

